Searching for Bumps in the Cosmological Road: Do Type Ia Supernovae with Early Excesses Have Biased Hubble Residuals?

Flux excesses in the early time light curves of Type Ia supernovae (SNe\,Ia) are predicted by multiple theoretical models and have been observed in a number of nearby SNe\,Ia over the last decade. However, the astrophysical processes that cause these excesses may affect their use as standardizable candles for cosmological parameter measurements. In this paper, we perform a systematic search for early-time excesses in SNe\,Ia observed by the Zwicky Transient Facility (ZTF) to study whether SNe\,Ia with these excesses yield systematically different Hubble residuals. We analyze two compilations of ZTF SN\,Ia light curves from its first year of operations: 127 high-cadence light curves from \citet{Yao19} and 305 light curves from the ZTF cosmology data release of \citet{Dhawan22}. We detect significant early-time excesses for 17 SNe\,Ia in these samples and find that the excesses have an average $g-r$ color of $0.06\pm0.09$~mag; we do not find a clear preference for blue excesses as predicted by several models. Using the SALT3 model, we measure Hubble residuals for these two samples and find that excess-having SNe\,Ia may have lower Hubble residuals (HR) after correcting for shape, color, and host-galaxy mass, at $\sim$2-3$\sigma$ significance; our baseline result is $\Delta HR = -0.056 \pm 0.026$~mag ($2.2 \sigma$). We compare the host-galaxy masses of excess-having and no-excess SNe\,Ia and find they are consistent, though at marginal significance excess-having SNe\,Ia may prefer lower-mass hosts. Additional discoveries of early excess SNe\,Ia will be a powerful way to understand potential biases in SN\,Ia cosmology and probe the physics of SN\,Ia progenitors.

==> old_tables.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| } 
  \hline
 
 SN & z & $t_{exp}$ & $x_0$ & $x_1$ & $c$ & $\Delta$ BIC & $f_{b, r}/f_{10, r}$ & $f_{b, g}/f_{10, g}$ &  $N$\\ 
 \hline
 \multicolumn{10}{|c|}{Gold Tier}\\
 \hline

 \hline
 \multicolumn{10}{|c|}{Bronze Tier} \\
 \hline
   2020ihr & 0.03 & 2458980.00 $\pm$ 0.02 & 3.45 $\pm 0.01 \times 10^{-3}$& -1.39 $\pm$ 0.02 & 0.007 $\pm$ 0.003 & 100 & 0.05 $\pm 0.04$ & 0.03 $\pm 0.02$ & 10\\ % chi2 is super high
2019mue & 0.041 & 2458715.24 $\pm$ 0.02 & 3.5 $\pm 0.01 \times 10^{-3}$ & -0.55 $\pm$ 0.02 & -0.038 $\pm$ 0.003 & 27 & 0.07 $\pm 0.04$ & 0.06 $\pm 0.04$ & 11 \\ %weird but there's definitely SOMETHING going on
  2020rtz & 0.03 & 2459095.90 $\pm$ 0.02 & 3.3 $\pm 0.02 \times 10^{-3}$ & -0.31 $\pm$ 0.03 & -0.0528 $\pm$ 0.004 & 6 & 0.04 $\pm 0.02$ & 0.03 $\pm 0.02$ & 10 \\ %looks pretty good
 2019hgw & 0.037 & 2458653.73 $\pm$ 0.02 & 2.042 $\pm 0.008 \times 10^{-3}$ & 0.55 $\pm$ 0.03 & 0.088 $\pm$ 0.03 & 1 & 0.03 $\pm 0.02$ & 0.02 $\pm 0.01$ & 10\\ %scatter is super high
 2019pdx & 0.02 & 2458741.14 $\pm$ 0.02 & 6.2 $\pm 0.02 \times 10^{-3}$ & -0.43 $\pm$ 0.02 & 0.049 $\pm$ 0.003 & -8 & 0.03 $\pm 0.02$ & 0.00 $\pm 0.02$& 10 \\ % very uncertain and only in red
 
 2019prw & 0.047 & 2458744.82 $\pm$ 0.04 & 1.26 $\pm 0.008 \times 10^{-3}$ & -2.72 $\pm$ 0.04 & 0.224 $\pm$ 0.006 & -2 & 0.04 $\pm 0.03$ & 0.0 $\pm 0.03$ & 10\\ %-- peak is measured wrong??
 2019rhx & 0.0254 & 2458767.02 $\pm$ 0.02 & 5.14 $\pm 0.02 \times 10^{-3}$ & -0.063 $\pm$ 0.03 & 0.069 $\pm$ 0.02 & 7 & 0.03 $\pm 0.03$ & 0.03 $\pm 0.02$ & 9\\ %very uncertain since there's not that much data in 5-10
 2019ubs & 0.034 & 2458806.81 $\pm 0.04$ & 3.85 $\pm 0.02 \times 10^{-3}$ & -0.48 $\pm 0.04$ & -0.026 $\pm 0.004$ & -8 & 0.02 $\pm 0.07$ & 0.02 $\pm 0.07$ & 9\\
 % 2020abdv -- bad data
 % 2020admb -- bad data
 
 %2020ilb just bad data tbh, no pre explosion data
 %2020qic actually a solid nondetection
 % 2020wcj bad data
 2020zpi & 0.037 & 2459182.38 $\pm$ 0.04 & 2.11 $\pm 0.01 \times 10^{-3}$ & 0.051 $\pm$ 0.05 $\pm $ & 0.147 $\pm$ 0.005 & 3 & 0.054 & 0.047 & 10\\ % very very narrow excess, 
 % 2021abko definitely not enough data
 % 2021rgw chi2 too high
 2021mwb & 0.043 & 2459370.51 $\pm$ 0.02 & 2.59 $\pm 0.005 \times 10^{-3}$ & 0.69 $\pm$ 0.02 & -0.002 $\pm$ 0.002 & 2 & 0.04 $\pm 0.05$ & 0.04 $\pm 0.05$ & 8 \\ %kind of weird but OK
 % 2021qve bad data
 % 2021qzn no bump
 2021xel & 0.04 & 2459472.15 $\pm$ 0.03 & 3.00 $\pm 0.01 \times 10^{-3}$ & 0.13 $\pm$ 0.03 & -0.031 $\pm$ 0.003 & 34 & 0.05 $\pm 0.04$& 0.04 $\pm 0.02$ & 11 \\ % pretty good
 \hline
 
 
 \hline
\end{tabular}
\caption{SN with early excesses and their SALT3 properties from the sample of ZTF 2019-2022 SN1a. Bump properties are quoted at reasonable, BIC-maximizing $N$. $f_b$ refers to the maximum excess bump flux, whereas $f_10$ refers to the flux at 10 days post-explosion, in each band.}
\end{table*}

==> suhail_52sec.tex <==
%% suggested section title renaming

Subsample comparison  and future improvements? 

%% 

While the \citet{Dhawan22} data were intended to be used for cosmological analyses, the ZTF forced-photometry data from \citet{Yao19} were not.  Despite this, the light-curve calibration appears to be sufficient to yield a Hubble-diagram scatter that is competitive with other recent cosmology samples, including \citet{Dhawan22}.

We note that there are two differences between the \citet{Yao19} and \citet{Dhawan22} samples. The first is that the $\beta$ parameter relating color to distance modulus is different at just under 3$\sigma$ significance between the two samples (Table \ref{table:tripp}).
%while the \citet{Yao19}-derived $\beta$ is closer to a Milky Way-like color law.  
This difference could be related to either sample selection effects or uncorrected calibration uncertainties in the 2018 ZTF photometry.

We note that both subsamples were derived with different photometric pipelines. While the \citet{Yao19} used the difference images from IPAC \citep[e.g., see][]{Masci19} and PSF photometry with \texttt{ForcedPhotZTF}, \citet{Dhawan22} construct custom template images and difference images and then used \texttt{photutils} \citep{larry_bradley_2023_7946442} for performing forced photometry. Given these differences in the processing,  we do not combine the photometric data, instead analyzing each self-consistent sample independently and use weighted averages to yield final constraints.

Secondly, the distance bias significantly differs between \citet{Yao19}-derived distances and those of \citet{Dhawan22}.  This is likely due to sample selection; while \citet{Dhawan22} started with a magnitude-limited sample and made additional cuts on host-galaxy redshift availability (thereby favoring bright host galaxies), \citet{Yao19} selected their sample based on the availability of high-S/N, high-cadence early-time light curves.  We attempt to marginalize over these differences by fitting a model to the redshift-dependent Hubble residuals and correcting for the trends, which are substantially different between the two data sets in this work.  This procedure is standard practice for SN\,Ia cosmology \citep[e.g.,][]{Marriner11}, but cosmology analyses also typically use large Monte Carlo simulations to estimate and correct for distance bias, which we have not performed here because it is not necessary for us to separate redshift-dependent Malmquist biases from differences in the cosmological model.  More complex evaluations of the distance bias will likely be performed by the ZTF team in the future, which could include pixel-level pipelines to model search and classification efficiencies and scene modelling photometry.
